$(\epsilon, u)$-Adaptive Regret Minimization in Heavy-Tailed Bandits

Heavy-tailed distributions naturally arise in several settings, from finance to telecommunications. While regret minimization under subgaussian or bounded rewards has been widely studied, learning with heavy-tailed distributions only gained popularity over the last decade. In this paper, we consider the setting in which the reward distributions have finite absolute raw moments of maximum order $1+\epsilon$, uniformly bounded by a constant $u<+\infty$, for some $\epsilon \in (0,1]$. In this setting, we study the regret minimization problem when $\epsilon$ and $u$ are unknown to the learner and it has to adapt. First, we show that adaptation comes at a cost and derive two negative results proving that the same regret guarantees of the non-adaptive case cannot be achieved with no further assumptions. Then, we devise and analyze a fully data-driven trimmed mean estimator and propose a novel adaptive regret minimization algorithm, AdaR-UCB, that leverages such an estimator. Finally, we show that AdaR-UCB is the first algorithm that, under a known distributional assumption, enjoys regret guarantees nearly matching those of the non-adaptive heavy-tailed case.

==> sections/05_experiments.tex <==
\section{Experimental Evaluation}
TODO

==> sections/old_02_setting.tex <==
% \section{Setting}
% We now introduce the stochastic heavy-tailed multi-armed bandit problem. Formally speaking, there are $K \ge 2$ available actions and a sequence of $T$ rounds. To each arm $i_t\in[K]$, we associate a probability distribution $\nu_i$ satisfying \eqref{eq:heavy-tail}. At each round $t\in[T]$, the agent can choose an index $i$ and  subsequently collects a reward of $X_t$, which is an independent sample from $\nu_i$. The agent is allowed to make a decision at round $t$ by considering all history up to time $t-1$. We remark that distributions $\{\nu_i\}_{i\in[K]}$ only admit finite moments up to order $1+\epsilon$, with $\epsilon \in (0, 1]$, thus distributions with infinite variance are allowed in this problem formulation. The goal of the agent is to minimize the regret as defined in \eqref{eq:regret}.
% In the heavy-tailed bandits literature, is customary to assume the knowledge on both $\epsilon$ and the upper bound on the $(1+\epsilon)$-th order moment $u$, which is assumed to be common for all $\{\nu_i\}_{i\in[K]}$ without loss of generality. The main contribution of this paper is twofold: first, we show that in general it is not possible to achieve the same order of performance of the state-of-the-art approaches while being unaware of these two quantities; then we propose an algorithm, called \algname (\algnameshort, for short), that under a specific distributional assumption called \textit{truncated non-positivty} is able to match the order of the regret lower bound for the classic scenario even when both $\epsilon$ and $u$ are unknown. Thus, in our setting, we will consider both quantities to be unknown to the agent. From now on, we will refer to any algorithm operating without this knowledge as \textit{adaptive w.r.t. $\epsilon$ or $u$}, depending on which one is unknown (possibly both).
